SAFE: Advancing Large Language Models in Leveraging Semantic and Syntactic Relationships for Software Vulnerability Detection

Software vulnerabilities (SVs) have emerged as a prevalent and critical concern for safety-critical security systems. This has spurred significant advancements in utilizing AI-based methods, including machine learning and deep learning, for software vulnerability detection (SVD). While AI-based methods have shown promising performance in SVD, their effectiveness on real-world, complex, and diverse source code datasets remains limited in practice. To tackle this challenge, in this paper, we propose a novel framework that enhances the capability of large language models to learn and utilize semantic and syntactic relationships from source code data for SVD. As a result, our approach can enable the acquisition of fundamental knowledge from source code data while adeptly utilizing crucial relationships, i.e., semantic and syntactic associations, to effectively address the software vulnerability detection (SVD) problem. The rigorous and extensive experimental results on three real-world challenging datasets (i.e., ReVeal, D2A, and Devign) demonstrate the superiority of our approach over the effective and state-of-the-art baselines. In summary, on average, our SAFE approach achieves higher performances from 4.79% to 9.15% for F1-measure and from 16.93% to 21.70% for Recall compared to the baselines across all datasets used.

==> sections/discussion.tex <==
\subsection{\textbf{Threats to validity }}

\paragraph{\textbf{Construct validity}}
Key construct validity threats are if the assessments of our proposed \ourapp~method and baselines demonstrate their capability for out-of-distribution source code data identification. In the cyber security domain, the out-of-distribution source code data identification task helps determine if an input is from an in-distribution (ID) or out-of-distribution (OOD). That enables the model and security experts to take appropriate precautions and actions. In particular, this stage assists security analysts and software engineers in identifying potential out-of-distribution CWE source code data outside the established in-distribution CWE source code data categories before feeding input data into subsequent machine learning and deep learning modules, to harden the software security systems. To evaluate the performance of our \ourapp~method and baselines, we use three main measures widely used in out-of-distribution detection including FPR (at TPR 95\%), AUROC, and AUPR.

\paragraph{\textbf{Internal validity}}
Key internal validity threats are relevant to the choice of hyper-parameter settings (i.e., optimizer, learning rate, number of layers in deep neural networks, etc.). It is worth noting that finding a set of optimal hyperparameter settings of deep neural networks is expensive due to a large number of trainable parameters. To train our method, we only use the common or default values for the hyperparameters. For example, we use the Adam optimizer; the learning rate equals $10^{-3}$; the size of neural layers is set in $\{100, 300\}$ while the scalar temperature $\tau$ used in the cluster-contrastive learning and the temperature $\nu$ for the Gumbel softmax distribution is set in $\{0.5, 1.0\}$. For the number of clusters used in cluster-contrastive learning aiming to improve the data representation learning process, we use it as a hyperparameter. In our paper, we detail the hyperparameter settings (i.e., the value-tuned ranges of the hyperparameters) in the released reproducible source code to support future replication studies.

\paragraph{\textbf{External validity}}
Key external validity threats include whether our \ourapp~method will generalize across multiple CWE source code categories. We mitigated this problem by conducting the experiments on an up-to-date and big C/C++ dataset.



==> tables/table3t.tex <==
\begin{table}[h]
\caption{The experimental results for Recall, Precision, and F1-measure of our approach when utilizing AST and DFG structures from the source code data. We denote our approach as \ourapp-R-AST and \ourapp-R-DFG when using RoBERTa as the backbone for the Student-S model with ASTs and DFGs for the Teacher-B model, respectively. Similarly, \ourapp-T-AST and \ourapp-T-DFG refer to our approach when using CodeT5 as the backbone for the Student-S model with ASTs and DFGs for the Teacher-B model, respectively.}\label{tab:astdfg}
\vspace{-1mm}
\centering{}
\resizebox{0.95\columnwidth}{!}{
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{ccccc}
\hline 
Datasets & Methods & Recall & Precision & F1-measure\tabularnewline
\hline 

%\multirow{2}{*}{Devign} & SODA-R-AST & 81.35\%  & \textbf{56.47\%} & 66.67\%\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
% & SODA-R-DFG & \textbf{85.82\%}  & 55.37\% & \textbf{67.31\%}\tabularnewline

\multirow{2}{*}{Devign} & \ourapp-R-AST & \textbf{81.35\%}  & 56.47\% & \textbf{66.67\%}\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 & \ourapp-R-DFG & 79.36\%  & \textbf{56.88\%} & 66.27\%\tabularnewline

\hline 

\multirow{2}{*}{ReVeal} & \ourapp-R-AST & \textbf{53.04\%}  & 37.65\% & \textbf{44.04\%}\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 & \ourapp-R-DFG & 44.35\%  & \textbf{40.64\%} & 42.41\%\tabularnewline
\hline 

\multirow{2}{*}{D2A} & \ourapp-R-AST & \textbf{89.29\%}  & 57.77\% & \textbf{70.15\%}\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 & \ourapp-R-DFG & 85.39\%  & \textbf{57.93\%} & 69.03\%\tabularnewline
\hline
\hline
\multirow{2}{*}{Devign} & \ourapp-T-AST & 78.73\%  & \textbf{57.61\%} & 66.53\%\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 & \ourapp-T-DFG & \textbf{80.16\%}  & 57.42\% & \textbf{66.91\%}\tabularnewline
\hline 

\multirow{2}{*}{ReVeal} & \ourapp-T-AST & 49.13\%  & \textbf{48.92\%}  & 49.02\%\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 & \ourapp-T-DFG & \textbf{52.40\%}  & 46.33\% & \textbf{49.18\%}\tabularnewline
\hline 

\multirow{2}{*}{D2A} & \ourapp-T-AST & 90.91\%  & \textbf{57.85\%} & \textbf{70.71\%}\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 & \ourapp-T-DFG & \textbf{91.56\% } & 56.06\% & 69.54\%\tabularnewline
\hline 
\end{tabular}}
\vspace{-2mm}
\end{table}

